JANUS: Agentic Cross-Language Fuzzing Harness Generation for Android Native Libraries

Modern Android apps extensively rely on native libraries, bridging Java/Kotlin and C/C++ through the Java Native Interface (JNI). This cross-language interoperation, however, exposes the memory-safe Android Runtime to the unsafe C/C++ world, creating an attack surface that has been repeatedly exploited for full device compromise. While fuzzing is a proven technique for vetting native libraries, state-of-the-art harness generation tools struggle to faithfully capture closed-source cross-language API usage: (i) precise program analysis across the JNI boundary does not scale, whereas lightweight approximations miss critical invocation patterns; and (ii) none tackles the construction of complex composite objects consumed by JNI methods. In this paper, we propose JANUS, the first agentic approach to synthesizing cross-language JNI-aware fuzzing harnesses for Android native libraries. JANUS iteratively resolves both explicit and implicit cross-language call dependencies to recover app-specific runtime context, and recursively assembles cross-language argument objects in a bottom-up manner. JANUS leverages an autonomous agentic workflow to reduce reliance on hand-crafted heuristics, capturing the vast landscape of hidden API usage knowledge embedded in closed-source native libraries. Evaluation on 44 popular real-world apps (such as Google and YouTube Music, covering 21,386 JNI methods total) shows that JANUS produces over 5.9 times as many valid harnesses (6,094) as state-of-the-art automatic harnessing tools. On pre-installed apps from five mainstream Android vendors (e.g., Xiaomi, Vivo, Samsung), JANUS further uncovers 6 previously unknown vulnerabilities in closed-source native libraries.

==> Makefile <==
SHELL := /bin/sh
.PHONY: all clean
all:
	@if command -v latexmk >/dev/null 2>&1; then \
	  latexmk -pdf -interaction=nonstopmode -halt-on-error main.tex; \
	elif command -v tectonic >/dev/null 2>&1; then \
	  tectonic --keep-logs --keep-intermediates main.tex; \
	elif test -x /opt/homebrew/bin/tectonic; then \
	  /opt/homebrew/bin/tectonic --keep-logs --keep-intermediates main.tex; \
	else \
	  printf '%s\n' 'Install TeX Live/MacTeX with latexmk, or Tectonic.'; exit 1; \
	fi
clean:
	rm -f main.aux main.blg main.fdb_latexmk main.fls main.log main.out main.synctex.gz

